Response-Time-Optimised Service Deployment: MILP Formulations of Piece-wise Linear Functions Approximating Non-linear Bivariate Mixed-integer Functions

A current trend in networking and cloud computing is to provide compute resources at widely dispersed places; this is exemplified by developments such as Network Function Virtualisation. This paves the way for wide-area service deployments with improved service quality: e.g, a nearby server can reduce the user-perceived response times. But always using the nearest server can be a bad decision if that server is already highly utilised. This paper formalises the two related problems of allocating resources at different locations and assigning users to them with the goal of minimising the response times for a given number of resources to use -- a non-linear capacitated facility location problem with integrated queuing systems. To efficiently handle the non-linearity, we introduce five linear problem approximations and adapt the currently best heuristic for a similar problem to our scenario. All six approaches are compared in experiments for solution quality and solving time. Surprisingly, our best optimisation formulation outperforms the heuristic in both time and quality. Additionally, we evaluate the influence ot resource distributions in the network on the response time: Cut by half for some configurations. The presented formulations are applicable to a broader optimisation domain.

==> documentProperties.tex <==
%
%
%
%
\RequirePackage[l2tabu, orthodox]{nag}

%
%
\newcommand{\ifdebug}[2]{ %
\ifthenelse{\isundefined{\mydebugmode}}{#2}{#1}
}

%
%
%
%
%

\usepackage{ifthen}
\usepackage{layouts}  % display various elements of a document's layout


%
%
%

\usepackage{graphicx}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{wrapfig}
\usepackage{rotfloat}
%
\graphicspath{{./fig/}}
\DeclareGraphicsExtensions{.pdf,.jpg,.jpeg,.png}
\usepackage{xcolor}
\usepackage{afterpage}

\usepackage{booktabs}
%
%



\usepackage{url}





%
%



%
%
%
%
%

\usepackage[ngerman, english]{babel}
\hyphenation{op-tical net-works semi-conduc-tor brain-strom-ing}
\usepackage[utf8]{inputenc}

%
%



%
%

%
%
%
%
%

%
%
%
	
	
%
%
\usepackage{enumitem}
  
  
%
%





%
%

\usepackage{amssymb, amsmath}
\allowdisplaybreaks  % split of large equation environments instead of move to next page
%
\usepackage{nicefrac}
\usepackage{units}
%


%
%
%
%
%
%
%
%
\usepackage{siunitx}
\sisetup{ 
    binary-units=true, % enables \byte and \gibi  
    per-mode = fraction,
    quotient-mode = fraction,
    fraction-function = \nicefrac, %
    decimalsymbol = {.}, %
    list-separator = {; },
    list-final-separator = {; },
    list-pair-separator = {; },
    list-units = single,  
    group-separator = {,} % enable ',' in 10,000
    %output-decimal-marker={,}% just uncomment if you want to use comma as the decimal marker!
}
\DeclareSIUnit\request{req.}
\DeclareSIUnit\req{\request}
\DeclareSIUnit\bps{bps.} %number of basepoints
\DeclareSIUnit\bit{bit}


\usepackage{algorithm}
\usepackage{algpseudocode}
%
\algtext*{EndWhile}
\algtext*{EndIf}
\algtext*{EndFor}
\algtext*{EndProcedure}
\algtext*{EndFunction}
\algrenewcommand\algorithmiccomment[1]{\hfill \textcolor{gray}{// #1}}
\algnewcommand\CommentLine[1]{\textcolor{gray}{/* #1 */}}

\usepackage{listings}
\lstset{ %
  basicstyle=\footnotesize,           % the size of the fonts that are used for the code
  numbers=left,                   % where to put the line-numbers
  numberstyle=\tiny\color{gray},  % the style that is used for the line-numbers
  stepnumber=2,                   % the step between two line-numbers. If it's 1, each line 
                                  % will be numbered
  numbersep=5pt,                  % how far the line-numbers are from the code
  captionpos=b,
}


\usepackage{amsthm}
\theoremstyle{definition}
\newtheorem{theorem}{Theorem}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%


	

%
%
%

%
%

\usepackage{newclude}
%
\usepackage{microtype}


%
\ifdebug{
	\usepackage[draft, inline]{showlabels} %left, outer, marginal
	\renewcommand{\showlabelfont}{ \footnotesize \sffamily\color{cyan} }
}{
    \usepackage[final]{showlabels} 
}




%
%
%

%
%
%




%


%
%
%
%
%

%
%


%
%
%
%
%
%
%
\usepackage[sort,compress]{cleveref}
\crefname{table}{table}{tables}
\crefname{figure}{figure}{figures}
\crefname{section}{section}{sections}
\crefname{chapter}{chapter}{chapters}
\crefname{lstlisting}{listing}{listings}
\crefname{requestthm}{request}{requests}
%
\crefname{equation}{}{}
\crefformat{equation}{(#2#1#3)} %#1#3} %##1##3}
\newcommand{\crefrangeconjunction}{--}
\crefformat{footnote}{#2\footnotemark[#1]#3} % this allow referencing a already referenced footnote with a label
\newcommand{\Coref}[1]{Constraint~\eqref{#1}}
\newcommand{\Transeq}[2]{\eqref{#1}${\rightarrow}$\eqref{#2}} % shortcut for (5)->(6)
\newcommand{\Lineref}[1]{Line~\ref{#1}}
   

   
%
%

\usepackage{float}
\floatstyle{ruled}
\newfloat{optproblem}{tbp}{}
\floatname{optproblem}{Optimisation Problem}
\crefname{optproblem}{Problem}{Problems}
   
 
%
%
%
%
%
   
\usepackage{setspace}

%
%
%

\ifdebug{
	\usepackage[inline,draft,index, multiuser,marginclue]{fixme}

}{
	\usepackage[final, multiuser]{fixme}
}


\FXRegisterAuthor{mk}{emk}{MK} % Matthias
\FXRegisterAuthor{hk}{ehk}{HK} % HK
\newcommand{\fmhkn}[1]{\hkwarning{#1}}
%
%
%

%
%
%





\usepackage{etoolbox}
\usepackage{comment}

\newcommand{\marker}[1]{\textcolor{black!80}{\fbox{\texttt{#1}}}\xspace} %\ensuremath{\mathfrak{#1}}
\newcommand{\markerbegin}[1]{\marker{#1{\small $\rightarrow$}}}
\newcommand{\markerend}[1]{\marker{{\small $\leftarrow$}#1}}
%
%
%


\ifdefmacro\extendedversion{
    \ifdefstring\extendedversion{draft}{
        % extendedversion == draft
        \newcommand{\ifextended}[2][]{%
            %\bgroup\color{black!80} [EXT]~#2~%
            %\ifstrempty{#1}{}{[NOEXT]~#1~}%
            %\bgroup \markerbegin{NOEXT}#2\markerend{NOEXT}%
            %\ifstrempty{#1}{}{\markerbegin{EXT}#1\markerend{EXT}}%            
            %\egroup}
            \ifstrempty{#1}{}{\markerbegin{EXT}#1\markerend{EXT}}%            
            \ifstrempty{#2}{}{\markerbegin{NOEXT}#2\markerend{NOEXT}}%
            }
               
        \newenvironment{inextended}[0] { %begin
                %\bgroup \color{black!80}[EXT]~%        
                \markerbegin{EXT}%        
            }{ %
                \markerend{EXT}}
            
        \newenvironment{notinextended}[0] { %begin
                %\bgroup \color{black!80}[NOEXT]~%        
                \markerbegin{NOEXT}%         
            }{ %
                \markerend{NOEXT}}
                               
    }{
    
        % extendedversion != draft
        \newcommand{\ifextended}[2][]{#2} %

        \excludecomment{notinextended}
        
        \newenvironment{inextended}[0] {}{}
    
    }

        
}{
    % not extendedversion 

    \newcommand{\ifextended}[2][]{#1}


    \excludecomment{inextended}
    
    \newenvironment{notinextended}[0] {}{}


}



%
%


%
%
%
%
%



%
%

\DeclareMathOperator*{\argmin}{arg\!min}
\DeclareMathOperator*{\argmax}{arg\!max}
\DeclareMathOperator*{\dom}{dom}

%


\usepackage{xspace}

\newcommand{\etal}[0]{~et~al.\@\xspace}
\newcommand{\etalcite}[1]{~et~al.~\cite{#1}\@\xspace}
\newcommand{\eg}{e.g.\@\xspace}
\newcommand{\etc}{etc.\@\xspace}
\newcommand{\ie}{i.e.\@\xspace}
\newcommand{\vs}{vs.\@\xspace}
\newcommand{\cf}{c.f.\@\xspace}

%
\newcommand{\lcf}{l_{cf}}
\newcommand{\xcf}{x_{cf}}
\newcommand{\zfs}{z_{fs}}
\newcommand{\Rn}{\mathbf{R}^n}
\newcommand{\Rnm}{\mathbf{R}^{n \times m}}
\newcommand{\Tamu}{T_{\mu_f} }



\newcommand\optP{\ensuremath{\mathsf{P}}\xspace}
\newcommand\optQP{\ensuremath{\mathsf{QP}}\xspace}
\newcommand\optQPx{\ensuremath{\mathsf{xQP}}\xspace}
\newcommand\optQPaiii{\ensuremath{\mathsf{cQP3}}\xspace}
\newcommand\optQPaii{\ensuremath{\mathsf{cQP2}}\xspace}
\newcommand\optQPai{\ensuremath{\mathsf{cQP1}}\xspace}
\newcommand\optQPa{\ensuremath{\mathsf{cQP}}\xspace}
\newcommand\optQPb[1][-]{\ensuremath{\mathsf{tQP}_{\hspace*{-0.7mm}#1}}\xspace}
\newcommand\optQPbb[1][+]{\ensuremath{\mathsf{tQP}_{\hspace*{-0.7mm}#1}}\xspace}
\newcommand\optQPc{\ensuremath{\mathsf{qQP}}\xspace}
\newcommand\optPABD{\ensuremath{\mathsf{QP}_{\hspace*{-0.7mm}\text{A}}}\xspace}

\newcommand\heu{\ensuremath{\mathsf{H}}\xspace}
\newcommand\funcEC{\ensuremath{\text{EC}}\xspace}
\newcommand\funcV{\ensuremath{\mathsf{V}}\xspace}
\newcommand\funcT[1][\mu]{\ensuremath{\mathsf{T}_{#1}}\xspace}
\newcommand\funcTa[1][\mu]{\ensuremath{\tilde{\mathsf{T}}_{#1}}\xspace}
\newcommand\funcTT[1][]{\ensuremath{\mathsf{T}#1}\xspace}
\newcommand\funcTTa[1][]{\ensuremath{\tilde{\mathsf{T}}#1}\xspace}
\newcommand\funcN[1][]{\ensuremath{\mathsf{N}}#1\xspace}
\newcommand\funcNa[1][]{\ensuremath{\tilde{\mathsf{N}}}#1\xspace}
\newcommand{\SetR}[1][\geq 0]{\mathbb{R}_{#1}}
\newcommand{\SetN}[1][\geq 0]{\mathbb{N}_{#1}}
\newcommand{\SetZ}[1][\geq 0]{\mathbb{Z}_{#1}}
\newcommand{\Pairv}{{v'\hspace{-.5mm}v}}
\newcommand{\Pairi}{{i'\hspace{-.5mm}i}}
\newcommand{\Pairc}{{c'\hspace{-.5mm}c}}


\newcommand{\sos}[1][2]{\ensuremath{\mathsf{SOS}#1}\xspace}

\newcommand\hG{\ensuremath{\hat G}\xspace}
\newcommand\hS{\ensuremath{\hat S}\xspace}
\newcommand\hD{\ensuremath{\hat D}\xspace}
\newcommand\hp{\ensuremath{\hat p}\xspace}
\newcommand\hAlgo{\ensuremath{\hat A}\xspace}
\newcommand\hTopo{\ensuremath{\hat T}\xspace}
\newcommand\hDem{\ensuremath{\hat D}\xspace}
\newcommand\hSer{\ensuremath{\hat S}\xspace}
\newcommand\hB{\ensuremath{\hat B}\xspace}
\newcommand\hLimit{\ensuremath{\hat p}\xspace}
\newcommand\hLam{\ensuremath{\hat \lambda}\xspace}
\newcommand\hMu{\ensuremath{\hat \mu}\xspace}


%
%

%


%
%







